Identification and Measurement of Technical Debt Requirements in Software Development: a Systematic Literature Review

Context: Technical Debt requirements are related to the distance between the ideal value of the specification and the system's actual implementation, which are consequences of strategic decisions for immediate gains, or unintended changes in context. To ensure the evolution of the software, it is necessary to keep it managed. Identification and measurement are the first two stages of the management process; however, they are little explored in academic research in requirements engineering. Objective: We aimed at investigating which evidence helps to strengthen the process of TD requirements management, including identification and measurement. Method: We conducted a Systematic Literature Review through manual and automatic searches considering 7499 studies from 2010 to 2020, and including 61 primary studies. Results: We identified some causes related to Technical Debt requirements, existing strategies to help in the identification and measurement, and metrics to support the measurement stage. Conclusion: Studies on TD requirements are still preliminary, especially on management tools. Yet, not enough attention is given to interpersonal issues, which are difficulties encountered when performing such activities, and therefore also require research. Finally, the provision of metrics to help measure TD is part of this work's contribution, providing insights into the application in the requirements context.

==> Table/PrimaryStudies.tex <==
\begin{table*} [pos=h]

\caption{Leading Causes Attributed to the Emergence of Technical Requirements Debt.}\label{Tab: PrimaryStudies}
\begin{tabular}{cl}
\hline
\textbf{ID} & \multicolumn{1}{c|}{\textbf{Primary Studies}}                                                                                                                                                                                                                                                                                                                       \\ \hline
P4                                                         & Hassouna, A., \& Tahvildari, L. (2010). An effort prediction framework for software defect correction. Information and Software Technology, 52(2), 197-209.                                                                                                                                                                                                         \\ \hline
P8                                                         & Guo, Y., \& Seaman, C. (2011, May). A portfolio approach to technical debt management. In Proceedings of the 2nd Workshop on Managing Technical Debt (pp. 31-34).                                                                                                                                                                                                   \\ \hline
P9                                                         & Klinger, T., Tarr, P., Wagstrom, P., \& Williams, C. (2011, May). An enterprise perspective on technical debt. In Proceedings of the 2nd Workshop on managing technical debt (pp. 35-38).                                                                                                                                                                           \\ \hline
P11                                                        & Theodoropoulos, T., Hofberg, M., \& Kern, D. (2011, May). Technical debt from the stakeholder perspective. In Proceedings of the 2nd Workshop on Managing Technical Debt (pp. 43-46).                                                                                                                                                                               \\ \hline
P13                                                        & Seaman, C., \& Guo, Y. (2011). Measuring and monitoring technical debt. In Advances in Computers (Vol. 82, pp. 25-46). Elsevier.                                                                                                                                                                                                                                    \\ \hline
P15                                                        & Nugroho, A., Visser, J., \& Kuipers, T. (2011, May). An empirical model of technical debt and interest. In Proceedings of the 2nd workshop on managing technical debt (pp. 1-8).                                                                                                                                                                                    \\ \hline
P23                                                        & Seaman, C., Guo, Y., Zazworka, N., Shull, F., Izurieta, C., Cai, Y., \& Vetrò, A. (2012, June). Using technical debt data in decision making: Potential decision approaches. In 2012 Third International Workshop on Managing Technical Debt (MTD) (pp. 45-48). IEEE.                                                                                               \\ \hline
P24                                                        & Snipes, W., Robinson, B., Guo, Y., \& Seaman, C. (2012, June). Defining the decision factors for managing defects: A technical debt perspective. In 2012 Third International Workshop on Managing Technical Debt (MTD) (pp. 54-60). IEEE.                                                                                                                           \\ \hline
P25                                                        & Ernst, N. A. (2012, June). On the role of requirements in understanding and managing technical debt. In 2012 Third International Workshop on Managing Technical Debt (MTD) (pp. 61-64). IEEE.                                                                                                                                                                       \\ \hline
P33                                                        & Curtis, B., Sappidi, J., \& Szynkarski, A. (2012, June). Estimating the size, cost, and types of technical debt. In 2012 Third International Workshop on Managing Technical Debt (MTD) (pp. 49-53). IEEE.                                                                                                                                                           \\ \hline
P34                                                        & Letouzey, J. L. (2012, June). The SQALE method for evaluating technical debt. In 2012 Third International Workshop on Managing Technical Debt (MTD) (pp. 31-36). IEEE.                                                                                                                                                                                              \\ \hline
P38                                                        & Spínola, R. O., Vetrò, A., Zazworka, N., Seaman, C., \& Shull, F. (2013, May). Investigating technical debt folklore: Shedding some light on technical debt opinion. In 2013 4th International Workshop on Managing Technical Debt (MTD) (pp. 1-7). IEEE.                                                                                                           \\ \hline
P43                                                        & Izurieta, C., Griffith, I., Reimanis, D., \& Luhr, R. (2013, June). On the uncertainty of technical debt measurements. In 2013 International Conference on Information Science and Applications (ICISA) (pp. 1-4). IEEE.                                                                                                                                            \\ \hline
P45                                                        & Zazworka, N., Spínola, R. O., Vetro', A., Shull, F., \& Seaman, C. (2013, April). A case study on effectively identifying technical debt. In Proceedings of the 17th International Conference on Evaluation and Assessment in Software Engineering (pp. 42-47).                                                                                                     \\ \hline
P49                                                        & Codabux, Z., \& Williams, B. (2013, May). Managing technical debt: An industrial case study. In 2013 4th International Workshop on Managing Technical Debt (MTD) (pp. 8-15). IEEE.                                                                                                                                                                                  \\ \hline
P50                                                        & Falessi, D., Shaw, M. A., Shull, F., Mullen, K., \& Keymind, M. S. (2013, May). Practical considerations, challenges, and requirements of tool-support for managing technical debt. In 2013 4th International Workshop on Managing Technical Debt (MTD) (pp. 16-19). IEEE.                                                                                          \\ \hline
P61                                                        & Sneed, H. M. (2014, January). Dealing with Technical Debt in agile development projects. In International Conference on Software Quality (pp. 48-62). Springer, Cham.                                                                                                                                                                                               \\ \hline
P72                                                        & Oliveira, F., Goldman, A., \& Santos, V. (2015, August). Managing technical debt in software projects using scrum: An action research. In 2015 Agile Conference (pp. 50-59). IEEE.                                                                                                                                                                                  \\ \hline
P74                                                        & Soares, H. F., Alves, N. S., Mendes, T. S., Mendonça, M., \& Spinola, R. O. (2015, April). Investigating the link between user stories and documentation debt on software projects. In 2015 12th International Conference on Information Technology-New Generations (pp. 385-390). IEEE.                                                                            \\ \hline
P76                                                        & \cellcolor[HTML]{FFF}Repaying Technical Debt in Practice                                                                                                                                                                                                                                                                                                            \\ \hline
P77                                                        & \cellcolor[HTML]{FFF}Tools for Repaying Technical Debt                                                                                                                                                                                                                                                                                                              \\ \hline
P79                                                        & Li, Z., Liang, P., \& Avgeriou, P. (2015, May). Architectural technical debt identification based on architecture decisions and change scenarios. In 2015 12th Working IEEE/IFIP Conference on Software Architecture (pp. 65-74). IEEE.                                                                                                                             \\ \hline
P81                                                        & Abad, Z. S. H., \& Ruhe, G. (2015, August). Using real options to manage technical debt in requirements engineering. In 2015 IEEE 23rd International Requirements Engineering Conference (RE) (pp. 230-235). IEEE.                                                                                                                                                  \\ \hline
P91                                                        & Mendes, T. S., de F. Farias, M. A., Mendonça, M., Soares, H. F., Kalinowski, M., \& Spínola, R. O. (2016, April). Impacts of agile requirements documentation debt on software projects: a retrospective study. In Proceedings of the 31st Annual ACM Symposium on Applied Computing (pp. 1290-1295).                                                               \\ \hline
P96                                                        & Martini, A., \& Bosch, J. (2016, May). An empirically developed method to aid decisions on architectural technical debt refactoring: AnaConDebt. In 2016 IEEE/ACM 38th International Conference on Software Engineering Companion (ICSE-C) (pp. 31-40). IEEE.                                                                                                       \\ \hline
P99                                                        & Akbarinasaji, S., Bener, A. B., \& Erdem, A. (2016, May). Measuring the principal of defect debt. In Proceedings of the 5th International Workshop on Realizing Artificial Intelligence Synergies in Software Engineering (pp. 1-7).                                                                                                                                \\ \hline
P101                                                       & Ghanbari, H. (2016, January). Seeking technical debt in critical software development projects: An exploratory field study. In 2016 49th Hawaii International Conference on System Sciences (HICSS) (pp. 5407-5416). IEEE.                                                                                                                                          \\ \hline
P110                                                       & Guo, Y., Spínola, R. O., \& Seaman, C. (2016). Exploring the costs of technical debt management–a case study. Empirical Software Engineering, 21(1), 159-182.                                                                                                                                                                                                       \\ \hline
P111                                                       & \cellcolor[HTML]{FFF}Yli-Huumo, J., Maglyas, A., \& Smolander, K. (2016). The Effects of Software Process Evolution to Technical Debt—Perceptions from Three Large Software Projects. In Managing Software Process Evolution (pp. 305-327). Springer, Cham.                                                                                                         \\ \hline
P117                                                       & Yli-Huumo, J., Maglyas, A., \& Smolander, K. (2016). How do software development teams manage technical debt?–An empirical study. Journal of Systems and Software, 120, 195-218.                                                                                                                                                                                    \\ \hline
P119                                                       & Ghanbari, H., Besker, T., Martini, A., \& Bosch, J. Looking for Peace of Mind? Manage your (Technical) Debt.                                                                                                                                                                                                                                                        \\ \hline
P125                                                       & Femmer, H., Fernández, D. M., Wagner, S., \& Eder, S. (2017). Rapid quality assurance with requirements smells. Journal of Systems and Software, 123, 190-213.                                                                                                                                                                                                      \\ \hline
P126                                                       & Mohagheghi, P., \& Aparicio, M. E. (2017). An industry experience report on managing product quality requirements in a large organization. Information and Software Technology, 88, 96-109.                                                                                                                                                                         \\ \hline
P132                                                       & Heikkilä, V. T., Paasivaara, M., Lasssenius, C., Damian, D., \& Engblom, C. (2017). Managing the requirements flow from strategy to release in large-scale agile development: a case study at Ericsson. Empirical Software Engineering, 22(6), 2892-2936.                                                                                                           \\ \hline
P133                                                       & Beer, A., Junker, M., Femmer, H., \& Felderer, M. (2017, September). Initial investigations on the influence of requirement smells on test-case design. In 2017 IEEE 25th International Requirements Engineering Conference Workshops (REW) (pp. 323-326). IEEE.                                                                                                    \\ \hline
P134                                                       & Femmer, H., Unterkalmsteiner, M., \& Gorschek, T. (2017, September). Which requirements artifact quality defects are automatically detectable? A case study. In 2017 IEEE 25th International Requirements Engineering Conference Workshops (REW) (pp. 400-406). IEEE.                                                                                               \\ \hline
P135                                                       & Ferrari, A., Spoletini, P., Donati, B., Zowghi, D., \& Gnesi, S. (2017, September). Interview review: detecting latent ambiguities to improve the requirements elicitation process. In 2017 IEEE 25th International Requirements Engineering Conference (RE) (pp. 400-405). IEEE.                                                                                   \\ \hline
P146                                                       & Ampatzoglou, A., Michailidis, A., Sarikyriakidis, C., Ampatzoglou, A., Chatzigeorgiou, A., \& Avgeriou, P. (2018, May). A framework for managing interest in technical debt: an industrial validation. In Proceedings of the 2018 International Conference on Technical Debt (pp. 115-124).                                                                         \\ \hline
P154                                                       & Charalampidou, S., Ampatzoglou, A., Chatzigeorgiou, A., \& Tsiridis, N. (2018, August). Integrating traceability within the ide to prevent requirements documentation debt. In 2018 44th Euromicro Conference on Software Engineering and Advanced Applications (SEAA) (pp. 421-428). IEEE.                                                                         \\ \hline
P158                                                       & Tsoukalas, D., Siavvas, M., Jankovic, M., Kehagias, D., Chatzigeorgiou, A., \& Tzovaras, D. (2018, September). Methods and Tools for TD Estimation and Forecasting: A State-of-the-art Survey. In 2018 International Conference on intelligent systems (IS) (pp. 698-705). IEEE.                                                                                    \\ \hline
P161                                                       & Conejero, J. M., Rodríguez-Echeverría, R., Hernández, J., Clemente, P. J., Ortiz-Caraballo, C., Jurado, E., \& Sánchez-Figueroa, F. (2018). Early evaluation of technical debt impact on maintainability. Journal of Systems and Software, 142, 92-114.                                                                                                             \\ \hline
P165                                                       & de O. Passos, A. F., de Freitas Farias, M. A., de Mendonça Neto, M. G., \& Spínola, R. O. (2018, October). A Study on Identification of Documentation and Requirement Technical Debt through Code Comment Analysis. In Proceedings of the 17th Brazilian Symposium on Software Quality (pp. 21-30).                                                                 \\ \hline
P167                                                       & Bano, M., Zowghi, D., Ferrari, A., Spoletini, P., \& Donati, B. (2018, August). Learning from mistakes: An empirical study of elicitation interviews performed by novices. In 2018 IEEE 26th International Requirements Engineering Conference (RE) (pp. 182-193). IEEE.                                                                                            \\ \hline
P171                                                       & Martini, A., Sikander, E., \& Madlani, N. (2018). A semi-automated framework for the identification and estimation of architectural technical debt: A comparative case-study on the modularization of a software component. Information and Software Technology, 93, 264-279.                                                                                       \\ \hline
P175                                                       & Conejero, J. M., Rodríguez-Echeverría, R., Hernández, J., Clemente, P. J., Ortiz-Caraballo, C., Jurado, E., \& Sánchez-Figueroa, F. (2018). Early evaluation of technical debt impact on maintainability. Journal of Systems and Software, 142, 92-114.                                                                                                             \\ \hline
P177                                                       & Kouros, P., Chaikalis, T., Arvanitou, E. M., Chatzigeorgiou, A., Ampatzoglou, A., \& Amanatidis, T. (2019, April). Jcaliper: search-based technical debt management. In Proceedings of the 34th ACM/SIGAPP Symposium on applied computing (pp. 1721-1730).                                                                                                          \\ \hline
P178                                                       & Rindell, K., Bernsmed, K., \& Jaatun, M. G. (2019, August). Managing Security in Software: Or: How I Learned to Stop Worrying and Manage the Security Technical Debt. In Proceedings of the 14th International Conference on Availability, Reliability and Security (pp. 1-8).                                                                                      \\ \hline
P183                                                       & Rios, N., Spínola, R. O., Mendonça, M., \& Seaman, C. (2019, May). Supporting analysis of technical debt causes and effects with cross-company probabilistic cause-effect diagrams. In 2019 IEEE/ACM International Conference on Technical Debt (TechDebt) (pp. 3-12). IEEE.                                                                                        \\ \hline
P192                                                       & Lenarduzzi, V., \& Fucci, D. (2019, September). Towards a holistic definition of requirements debt. In 2019 ACM/IEEE International Symposium on Empirical Software Engineering and Measurement (ESEM) (pp. 1-5). IEEE.                                                                                                                                              \\ \hline
P196                                                       & Mendes, T. S., Gomes, F. G., Gonçalves, D. P., Mendonça, M. G., Novais, R. L., \& Spínola, R. O. (2019). VisminerTD: a tool for automatic identification and interactive monitoring of the evolution of technical debt items. Journal of the Brazilian Computer Society, 25(1), 1-28.                                                                               \\ \hline
P203                                                       & Freire, S., Rios, N., Mendonça, M., Falessi, D., Seaman, C., Izurieta, C., \& Spínola, R. O. (2020, March). Actions and impediments for technical debt prevention: results from a global family of industrial surveys. In Proceedings of the 35th Annual ACM Symposium on Applied Computing (pp. 1548-1555).                                                        \\ \hline
P208                                                       & Freire, S., Rios, N., Gutierrez, B., Torres, D., Mendonça, M., Izurieta, C., ... \& Spínola, R. O. (2020). Surveying software practitioners on technical debt payment practices and reasons for not paying off debt items. In Proceedings of the Evaluation and Assessment in Software Engineering (pp. 210-219).                                                   \\ \hline
P209                                                       & Behutiye, W., Seppänen, P., Rodríguez, P., \& Oivo, M. (2020). Documentation of quality requirements in agile software development. In Proceedings of the Evaluation and Assessment in Software Engineering (pp. 250-259).                                                                                                                                          \\ \hline
P214                                                       & Behutiye, W., Rodríguez, P., Oivo, M., Aaramaa, S., Partanen, J., \& Abhervé, A. (2020, August). How agile software development practitioners perceive the need for documenting quality requirements: a multiple case study. In 2020 46th Euromicro Conference on Software Engineering and Advanced Applications (SEAA) (pp. 93-100). IEEE.                         \\ \hline
P216                                                       & Li, Y., Soliman, M., \& Avgeriou, P. (2020, August). Identification and Remediation of Self-Admitted Technical Debt in Issue Trackers. In 2020 46th Euromicro Conference on Software Engineering and Advanced Applications (SEAA) (pp. 495-503). IEEE.                                                                                                              \\ \hline
P225                                                       & \cellcolor[HTML]{FFF}On the   Perceived Harmfulness of Requirement Smells: An Empirical Study                                                                                                                                                                                                                                                                       \\ \hline
P228                                                       & Besker, T., Ghanbari, H., Martini, A., \& Bosch, J. (2020). The influence of Technical Debt on software developer morale. Journal of Systems and Software, 167, 110586.                                                                                                                                                                                             \\ \hline
P229                                                       & Rios, N., Spínola, R. O., Mendonça, M., \& Seaman, C. (2020). The practitioners’ point of view on the concept of technical debt and its causes and consequences: a design for a global family of industrial surveys and its first results from Brazil. Empirical Software Engineering, 25(5), 3216-3287.                                                            \\ \hline
P233                                                       & de Freitas Farias, M. A., de Mendonça Neto, M. G., Kalinowski, M., \& Spínola, R. O. (2020). Identifying self-admitted technical debt through code comment analysis with a contextualized vocabulary. Information and Software Technology, 121, 106270.                                                                                                             \\ \hline
P247                                                       & Dar, H. S. (2020, August). Reducing Ambiguity in Requirements Elicitation via Gamification. In 2020 IEEE 28th International Requirements Engineering Conference (RE) (pp. 440-444). IEEE.                                                                                                                                                                           \\ \hline
P249                                                       & Panis, M. C. (2020, August). An Analysis of Requirements-Related Problems that Occurred in an organization Using a Mature Requirements Engineering Process. In 2020 IEEE 28th International Requirements Engineering Conference (RE) (pp. 291-299). IEEE.                                                                                                           \\ \hline
P258                                                       & Curtis, B., Sappidi, J., \& Szynkarski, A. (2012). Estimating the principal of an application's technical debt. IEEE software, 29(6), 34-42.                                                                                                                                                                                                                        \\ \hline
P263                                                       & Femmer, H., Fernández, D. M., Juergens, E., Klose, M., Zimmer, I., \& Zimmer, J. (2014, June). Rapid requirements checks with requirements smells: Two case studies. In Proceedings of the 1st International Workshop on Rapid Continuous Software Engineering (pp. 10-19).                                                                                         \\ \hline
P273                                                       & Robiolo, G., Scott, E., Matalonga, S., \& Felderer, M. (2019, November). Technical debt and waste in non-functional requirements documentation: An exploratory study. In International Conference on Product-Focused Software Process Improvement (pp. 220-235). Springer, Cham.                                                                                    \\ \hline
P274                                                       & Lenarduzzi, V., Orava, T., Saarimäki, N., Systa, K., \& Taibi, D. (2019, September). An empirical study on technical debt in a finnish sme. In 2019 ACM/IEEE International Symposium on Empirical Software Engineering and Measurement (ESEM) (pp. 1-6). IEEE.                                                                                                      \\ \hline
P275                                                       & Rios, N., Mendes, L., Cerdeiral, C., Magalhães, A. P. F., Perez, B., Correal, D., ... \& Spínola, R. O. (2020, March). Hearing the voice of software practitioners on causes, effects, and practices to Deal with documentation debt. In International Working Conference on Requirements Engineering: Foundation for Software Quality (pp. 55-70). Springer, Cham. \\ \hline
\end{tabular}
\end{table*}

==> Table/studies.tex <==
\begin{table}[pos=h]
\label{studies}
\begin{tabular}{{p{0.23in}p{2.8in}}}
\hline
\textbf{{[}P4{]}}  & \begin{tabular}[c]{@{}l@{}}An effort prediction framework for software defect\\correction.\end{tabular}                                        \\ 
\textbf{{[}P8{]}}  & A portfolio approach to technical debt management.                                                                                              \\ 
\textbf{{[}P9{]}}  & An enterprise perspective on technical debt.                                                                                                    \\ 
\textbf{{[}P11{]}} & Technical debt from the stakeholder perspective.                                                                                                \\ 
\textbf{{[}P13{]}} & Measuring and monitoring technical debt.                                                                                                        \\ 
\textbf{{[}P15{]}} & An empirical model of technical debt and interest.                                                                                              \\ 
\textbf{{[}P23{]}} & \begin{tabular}[c]{@{}l@{}}Using technical debt data in decision making:\\ Potential decision approaches.\end{tabular}                          \\ 
\textbf{{[}P24{]}} & \begin{tabular}[c]{@{}l@{}}Defining the decision factors for managing defects:\\ a technical debt perspective.\end{tabular}                     \\ 
\textbf{{[}P25{]}} & \begin{tabular}[c]{@{}l@{}}On the role of requirements in understanding and\\ managing technical debt.\end{tabular}                             \\ 
\textbf{{[}P33{]}} & \begin{tabular}[c]{@{}l@{}}Estimating the size, cost, and types of technical debt.\end{tabular}                                               \\ 
\textbf{{[}P34{]}} & The SQALE method for evaluating technical debt.                                                                                                 \\ 
\textbf{{[}P38{]}} & \begin{tabular}[c]{@{}l@{}}Investigating technical debt folklore: Shedding\\ some light on technical debt opinion.\end{tabular}                 \\ 
%\textbf{{[}P39{]}} & \begin{tabular}[c]{@{}l@{}}DebtFlag: Technical debt management with a\\ development environment integrated tool.\end{tabular}                   \\ 
\textbf{{[}P43{]}} & On the uncertainty of technical debt measurements.                                                                                              \\ 
\textbf{{[}P45{]}} & \begin{tabular}[c]{@{}l@{}}A case study on effectively identifying technical debt.\end{tabular}                                               \\ 
\textbf{{[}P49{]}} & Managing technical debt: An industrial case study.                                                                                              \\ 
\textbf{{[}P50{]}} & \begin{tabular}[c]{@{}l@{}}Practical considerations, challenges and requirements\\ of tool-support for managing technical debt.\end{tabular} \\ 
\textbf{{[}P61{]}} & \begin{tabular}[c]{@{}l@{}}Dealing with Technical Debt in agile development\\ projects.\end{tabular}                                            \\ 
\textbf{{[}P72{]}} & \begin{tabular}[c]{@{}l@{}}Managing technical debt in software projects using\\ scrum: An action research.\end{tabular}                         \\ 
\textbf{{[}P74{]}} & \begin{tabular}[c]{@{}l@{}}Investigating the link between user stories and\\ documentation debt on software projects.\end{tabular}              \\ 
\textbf{{[}P76{]}} & Repaying technical debt in practice.                                                                                                            \\ 
\textbf{{[}P77{]}} & Tools for repaying technical debt.    \\
\textbf{{[}P79{]}} & \begin{tabular}[c]{@{}l@{}}Architectural technical debt identification based on\\ architecture decisions and change scenarios.\end{tabular}         \\ 
\textbf{{[}P81{]}} & \begin{tabular}[c]{@{}l@{}}Using real options to manage technical debt in\\ requirements engineering.\end{tabular}                                  \\ 
\textbf{{[}P91{]}} & \begin{tabular}[c]{@{}l@{}}Impacts of agile requirements documentation debt\\ on software projects: a retrospective study.\end{tabular}             \\ 
%\textbf{{[}P92{]}} & \begin{tabular}[c]{@{}l@{}}Tool support for evaluating architectural debt of an\\ existing system: An experience report.\end{tabular}               \\ 
\textbf{{[}P96{]}} & \begin{tabular}[c]{@{}l@{}}An empirically developed method to aid decisions on\\ architectural technical debt refactoring: AnaConDebt.\end{tabular} \\ 
\textbf{{[}P99{]}}  & Measuring the principal of defect debt.                                                                                   \\ 
\textbf{{[}P101{]}} & \begin{tabular}[c]{@{}l@{}}Seeking technical debt in critical software\\ development projects: An exploratory field study.\end{tabular}                                                                             \\
\textbf{{[}P110{]}} & Exploring the costs of technical debt management–a \newline case study.  \\                                                 \textbf{{[}P111{]}} & \begin{tabular}[c]{@{}l@{}}The Effects of Software Process Evolution to\\ Technical Debt — Perceptions from Three Large\\ Software Projects.\end{tabular} 
\\
\textbf{{[}P117{]}} & \begin{tabular}[c]{@{}l@{}}How do software development teams manage\\ technical debt? – An empirical study.\end{tabular} 
\\
\textbf{{[}P119{]}}  & Looking for peace of mind? manage your (technical) \newline debt: An exploratory field study.           
\\
\textbf{{[}P125{]}}  & Rapid quality assurance with requirements smells. 
\end{tabular}
\end{table}

==> Table/studies2.tex <==
\begin{table}[pos=h]
\label{studies2}
\begin{tabular}{{p{0.23in}p{2.8in}}}
 
\textbf{{[}P126{]}}  & \begin{tabular}[c]{@{}l@{}}An industry experience report on managing product\\ quality requirements in a large organization.\end{tabular}                                                                           \\ 
%\textbf{{[}P128{]}}  & \begin{tabular}[c]{@{}l@{}}The pricey bill of technical debt: When and by whom\\ will it be paid?.\end{tabular}                                                                                                     \\ 
\textbf{{[}P132{]}}  & \begin{tabular}[c]{@{}l@{}}Managing the requirements flow from strategy to\\ release in large-scale agile development: a case study\\ at Ericsson.\end{tabular}                                                       \\ 
\textbf{{[}P133{]}}  & \begin{tabular}[c]{@{}l@{}}Initial investigations on the influence of requirement\\ smells on test-case design.\end{tabular}                                                                                        \\ 
\textbf{{[}P134{]}}  & \begin{tabular}[c]{@{}l@{}}Which requirements artifact quality defects are\\ automatically detectable? A case study.\end{tabular}                                                                                   \\ 
\textbf{{[}P135{]}}  & \begin{tabular}[c]{@{}l@{}}Interview review: detecting latent ambiguities to\\ improve the requirements elicitation process.\end{tabular}                         \\ 
%\textbf{{[}P143{]}} & \begin{tabular}[c]{@{}l@{}}Limiting technical debt with maintainability assurance:\\ an industry survey on used techniques and differences\\ with service-and microservice-based systems.\end{tabular}              \\
\textbf{{[}P146{]}} & \begin{tabular}[c]{@{}l@{}}A framework for managing interest in technical debt:\\ an industrial validation.\end{tabular}                                           \\
%\textbf{{[}P148{]}} & \begin{tabular}[c]{@{}l@{}}Technical debt cripples software developer productivity:\\ a longitudinal study on developers' daily software\\ development work.\end{tabular}                                           \\ 
\textbf{{[}P154{]}} & \begin{tabular}[c]{@{}l@{}}Integrating Traceability within the IDE to Prevent \\ Requirements Documentation Debt.\end{tabular}                                     \\ 
\textbf{{[}P158{]}} & \begin{tabular}[c]{@{}l@{}}Methods and Tools for TD Estimation and Forecasting:\\ A State-of-the-art Survey.\end{tabular}                                        \\ 
\textbf{{[}P161{]}} & Early evaluation of technical debt impact on maintainability.                                           \\ 
%\textbf{{[}P163{]}} & \begin{tabular}[c]{@{}l@{}}Technical Debt tracking: Current state of practice:\\ A survey and multiple case study in 15 large\\ organizations.\end{tabular}                                                           \\ 
\textbf{{[}P165{]}} & \begin{tabular}[c]{@{}l@{}}A Study on Identification of Documentation and\\ Requirement Technical Debt through Code Comment\\ Analysis.\end{tabular}                                                                  \\ 
\textbf{{[}P167{]}} & \begin{tabular}[c]{@{}l@{}}Learning from mistakes: An empirical study of\\ elicitation interviews performed by novices.\end{tabular}                                                                                \\ 
\textbf{{[}P171{]}} & \begin{tabular}[c]{@{}l@{}}A semi-automated framework for the identification\\ and estimation of architectural technical debt:\\ comparative case-study on the modularization of a\\ software component.\end{tabular} \\ 
\textbf{{[}P175{]}} & Early evaluation of technical debt impact on maintainability.        \\                                         \textbf{{[}P177{]}} & JCaliper: search-based technical debt management.                                                                \\ 
\textbf{{[}P178{]}} & Managing Security in Software.                                                                                   \\ 
\textbf{{[}P183{]}} & \begin{tabular}[c]{@{}l@{}}Supporting analysis of technical debt causes and\\ effects with cross-company probabilistic\\ cause-effect diagrams.\end{tabular}                                                          \\ 
\textbf{{[}P192{]}} & Towards a holistic definition of requirements debt.  \\            \textbf{{[}P196{]}} & \begin{tabular}[c]{@{}l@{}}VisminerTD: a tool for automatic identification and\\ interactive monitoring of the evolution of technical\\ debt items.\end{tabular}                           \hline                        
\end{tabular}
\end{table}
